Attention-based Fusion for Multi-source Human Image Generation

We present a generalization of the person-image generation task, in which a human image is generated conditioned on a target pose and a set X of source appearance images. In this way, we can exploit multiple, possibly complementary images of the same person which are usually available at training and at testing time. The solution we propose is mainly based on a local attention mechanism which selects relevant information from different source image regions, avoiding the necessity to build specific generators for each specific cardinality of X. The empirical evaluation of our method shows the practical interest of addressing the person-image generation problem in a multi-source setting.

==> fashionSup2.tex <==
\begin{figure*}[h]
   \centering
   \setlength\tabcolsep{1.0pt}
   \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc|c}
     %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
     $x^i,i\in[1..3]$ & $x_\tau$ & $M_n=2$ & $M_n=3$ & $M_n=4$&  \small Attention Saliency\\ 

\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000300206_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000300206_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000300206_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000300206_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000300206_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000300206_4full.png}
\\
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENDressesid0000409106_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENDressesid0000409106_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENDressesid0000409106_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENDressesid0000409106_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENDressesid0000409106_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENDressesid0000409106_1front.png}
%% \\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000660212_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000660212_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000660212_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000660212_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000660212_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000660212_2side.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENSweatersid0000084004_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENSweatersid0000084004_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENSweatersid0000084004_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENSweatersid0000084004_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENSweatersid0000084004_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENSweatersid0000084004_2side.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000512402_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000512402_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000512402_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000512402_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000512402_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000512402_3back.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENDressesid0000766701_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENDressesid0000766701_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENDressesid0000766701_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENDressesid0000766701_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENDressesid0000766701_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENDressesid0000766701_4full.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENDressesid0000528102_1front.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENDressesid0000528102_1front.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENDressesid0000528102_1front.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENDressesid0000528102_1front.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENDressesid0000528102_1front.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENDressesid0000528102_1front.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENBlousesShirtsid0000299703_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENBlousesShirtsid0000299703_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENBlousesShirtsid0000299703_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENBlousesShirtsid0000299703_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENBlousesShirtsid0000299703_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENBlousesShirtsid0000299703_3back.png}
\\

 \end{tabular}}
   \vspace{-0.4cm} 
  \caption{} 
  \end{figure*}


\begin{figure*}[h]
   \centering
   \setlength\tabcolsep{1.0pt}
   \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc|c}
     %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
     $x^i,i\in[1..2]$ & $x_\tau$ & $M_n=2$ & $M_n=3$ & $M_n=4$&  \small Attention Saliency\\ 
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000216220_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000216220_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000216220_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000216220_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000216220_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000216220_3back.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENDressesid0000648602_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENDressesid0000648602_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENDressesid0000648602_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENDressesid0000648602_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENDressesid0000648602_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENDressesid0000648602_2side.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000629705_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000629705_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000629705_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000629705_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000629705_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000629705_2side.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionMENTeesTanksid0000663402_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionMENTeesTanksid0000663402_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionMENTeesTanksid0000663402_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionMENTeesTanksid0000663402_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionMENTeesTanksid0000663402_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionMENTeesTanksid0000663402_4full.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000296910_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000296910_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000296910_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000296910_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000296910_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000296910_2side.png}
\\

 \end{tabular}}
   \vspace{-0.4cm} 
  \caption{Failure cases on the DeepFashion dataset.}
\label{fig:failures}
\end{figure*}



==> fashionSupAblation.tex <==
\begin{figure*}[h]
   \centering
   \setlength\tabcolsep{1.0pt}
   \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc|c}
     %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
     $x^i,i\in[1..3]$ & $x_\tau$ & \emph{Avg}& \emph{Full}&  \small Attention Saliency\\ 

\includegraphics[height=0.24\columnwidth]{./figures/sup/full/input_fasionWOMENBlousesShirtsid0000128902_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/GT_fasionWOMENBlousesShirtsid0000128902_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/avg/fasionWOMENBlousesShirtsid0000128902_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/fasionWOMENBlousesShirtsid0000128902_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/att_fasionWOMENBlousesShirtsid0000128902_7additional.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/input_fasionWOMENBlousesShirtsid0000546602_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/GT_fasionWOMENBlousesShirtsid0000546602_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/avg/fasionWOMENBlousesShirtsid0000546602_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/fasionWOMENBlousesShirtsid0000546602_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/att_fasionWOMENBlousesShirtsid0000546602_4full.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/input_fasionWOMENCardigansid0000369601_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/GT_fasionWOMENCardigansid0000369601_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/avg/fasionWOMENCardigansid0000369601_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/fasionWOMENCardigansid0000369601_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/att_fasionWOMENCardigansid0000369601_4full.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/input_fasionMENShirtsPolosid0000541703_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/GT_fasionMENShirtsPolosid0000541703_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/avg/fasionMENShirtsPolosid0000541703_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/fasionMENShirtsPolosid0000541703_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/att_fasionMENShirtsPolosid0000541703_4full.png}
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/full/input_fasionMENJacketsVestsid0000016802_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/full/GT_fasionMENJacketsVestsid0000016802_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/avg/fasionMENJacketsVestsid0000016802_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/full/fasionMENJacketsVestsid0000016802_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/full/att_fasionMENJacketsVestsid0000016802_1front.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/input_fasionWOMENTeesTanksid0000311404_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/GT_fasionWOMENTeesTanksid0000311404_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/avg/fasionWOMENTeesTanksid0000311404_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/fasionWOMENTeesTanksid0000311404_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/att_fasionWOMENTeesTanksid0000311404_3back.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/input_fasionWOMENBlousesShirtsid0000409003_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/GT_fasionWOMENBlousesShirtsid0000409003_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/avg/fasionWOMENBlousesShirtsid0000409003_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/fasionWOMENBlousesShirtsid0000409003_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/full/att_fasionWOMENBlousesShirtsid0000409003_3back.png}

%% \\

%% \includegraphics[height=0.24\columnwidth]{./figures/sup/full/input_fasionMENJacketsVestsid0000333606_3back.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/full/GT_fasionMENJacketsVestsid0000333606_3back.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/avg/fasionMENJacketsVestsid0000333606_3back.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/full/fasionMENJacketsVestsid0000333606_3back.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/full/att_fasionMENJacketsVestsid0000333606_3back.png}
%% \\
 \end{tabular}}
   \vspace{-0.4cm} 
  \caption{Additional qualitative comparison between  \emph{Avg} and \emph{Full}  on the DeepFashion dataset.}\label{fig:abl} 
  \end{figure*}


==> fashionSupFailures.tex <==


\begin{figure*}[h]
   \centering
   \setlength\tabcolsep{1.0pt}
   \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc|c}
     %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
     $x^i,i\in[1..3]$ & $x_\tau$ & $M_n=2$ & $M_n=3$ & $M_n=4$&  \small Attention Saliency\\ 
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000216220_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000216220_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000216220_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000216220_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000216220_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000216220_3back.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENDressesid0000648602_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENDressesid0000648602_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENDressesid0000648602_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENDressesid0000648602_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENDressesid0000648602_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENDressesid0000648602_2side.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000629705_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000629705_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000629705_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000629705_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000629705_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000629705_2side.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionMENTeesTanksid0000663402_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionMENTeesTanksid0000663402_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionMENTeesTanksid0000663402_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionMENTeesTanksid0000663402_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionMENTeesTanksid0000663402_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionMENTeesTanksid0000663402_4full.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000296910_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000296910_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000296910_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000296910_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000296910_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000296910_2side.png}
\\

 \end{tabular}}
   \vspace{-0.4cm} 
  \caption{Some {\em failure} cases on the DeepFashion dataset.}
  \label{fig:DeepFashionfailures}
  \end{figure*}



==> fashionSupVarying.tex <==

\begin{figure*}[h]
   \centering
   \setlength\tabcolsep{1.0pt}
   \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc}
     %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
     $x^i,i\in[1..4]$ & $x_\tau$ & $M_n=2$ & $M_n=3$ & $M_n=4$ \\% & \small Attention Saliency\\ 
\includegraphics[height=0.24\columnwidth]{./figures/full_4/input_fasionMENJacketsVestsid0000333606_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/GT_fasionMENJacketsVestsid0000333606_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_2/fasionMENJacketsVestsid0000333606_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_3/fasionMENJacketsVestsid0000333606_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/fasionMENJacketsVestsid0000333606_3back.png}\\
\includegraphics[height=0.24\columnwidth]{./figures/full_4/input_fasionMENTeesTanksid0000404701_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/GT_fasionMENTeesTanksid0000404701_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_2/fasionMENTeesTanksid0000404701_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_3/fasionMENTeesTanksid0000404701_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/fasionMENTeesTanksid0000404701_3back.png}\\

%\includegraphics[height=0.24\columnwidth]{./figures/full_4/att_fasionMENJacketsVestsid0000333606_3back.png}\\
\includegraphics[height=0.24\columnwidth]{./figures/full_4/input_fasionWOMENCardigansid0000052102_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/GT_fasionWOMENCardigansid0000052102_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_2/fasionWOMENCardigansid0000052102_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_3/fasionWOMENCardigansid0000052102_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/fasionWOMENCardigansid0000052102_2side.png}\\
%\includegraphics[height=0.24\columnwidth]{./figures/full_4/att_fasionWOMENCardigansid0000052102_2side.png}\\ 


%\includegraphics[height=0.24\columnwidth]{./figures/full_4/att_fasionWOMENTeesTanksid0000296910_2side.png}\\


\includegraphics[height=0.24\columnwidth]{./figures/full_4/input_fasionWOMENBlousesShirtsid0000548203_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/GT_fasionWOMENBlousesShirtsid0000548203_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_2/fasionWOMENBlousesShirtsid0000548203_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_3/fasionWOMENBlousesShirtsid0000548203_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/fasionWOMENBlousesShirtsid0000548203_3back.png}\\

%\includegraphics[height=0.24\columnwidth]{./figures/full_4/att_fasionWOMENBlousesShirtsid0000548203_2side.png}\\
\includegraphics[height=0.24\columnwidth]{./figures/full_4/input_fasionWOMENBlousesShirtsid0000763402_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/GT_fasionWOMENBlousesShirtsid0000763402_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_2/fasionWOMENBlousesShirtsid0000763402_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_3/fasionWOMENBlousesShirtsid0000763402_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/fasionWOMENBlousesShirtsid0000763402_7additional.png}\\
%\includegraphics[height=0.24\columnwidth]{./figures/full_4/att_fasionWOMENBlousesShirtsid0000763402_2side.png}\\
%% \includegraphics[height=0.24\columnwidth]{./figures/full_4/input_fasionWOMENJacketsCoatsid0000018710_4full.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/full_4/GT_fasionWOMENJacketsCoatsid0000018710_4full.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/full_2/fasionWOMENJacketsCoatsid0000018710_4full.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/full_3/fasionWOMENJacketsCoatsid0000018710_4full.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/full_4/fasionWOMENJacketsCoatsid0000018710_4full.png}\\
%% \includegraphics[height=0.24\columnwidth]{./figures/full_4/input_fasionWOMENJacketsCoatsid0000018710_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/full_4/GT_fasionWOMENJacketsCoatsid0000018710_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/full_2/fasionWOMENJacketsCoatsid0000018710_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/full_3/fasionWOMENJacketsCoatsid0000018710_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/full_4/fasionWOMENJacketsCoatsid0000018710_1front.png}
\includegraphics[height=0.24\columnwidth]{./figures/full_4/input_fasionWOMENJacketsCoatsid0000018710_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/GT_fasionWOMENJacketsCoatsid0000018710_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_2/fasionWOMENJacketsCoatsid0000018710_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_3/fasionWOMENJacketsCoatsid0000018710_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/full_4/fasionWOMENJacketsCoatsid0000018710_7additional.png}

%\includegraphics[height=0.24\columnwidth]{./figures/full_4/att_fasionWOMENSweatersid0000112302_1front.png}\\ 

 \end{tabular}}
   \vspace{-0.4cm} 
   \caption{Qualitative evaluation on the DeepFashion Dataset of a model {\em trained} with $M_n=2$ and then {\em tested} with varying $M_n$ values (from 2 to 4). The first 4 columns show the {\em testing} source images 
which correspond to the last 3 columns showing the generated images. For instance, the first 2 columns correspond to testing with  $M_n = 2$  sources, whose result is shown in the corresponding column; while
 the first 3 columns correspond to testing with  $M_n = 3$  sources, etc.}
%  from left to right  to the testing $\Xvect_n$.}
   \label{fig:qualVarying}
  \end{figure*}


==> fashionsupadditional.tex <==
\begin{figure*}[h]
   \centering
   \setlength\tabcolsep{1.0pt}
   \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc|c}
     %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
     $x^i,i\in[1..3]$ & $x_\tau$ & $M_n=1$ & $M_n=2$ & $M_n=3$&  \small Attention Saliency\\ 

\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000300206_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000300206_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000300206_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000300206_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000300206_4full.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000300206_4full.png}
\\
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENDressesid0000409106_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENDressesid0000409106_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENDressesid0000409106_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENDressesid0000409106_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENDressesid0000409106_1front.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENDressesid0000409106_1front.png}
%% \\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000660212_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000660212_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000660212_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000660212_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000660212_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000660212_2side.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENSweatersid0000084004_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENSweatersid0000084004_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENSweatersid0000084004_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENSweatersid0000084004_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENSweatersid0000084004_2side.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENSweatersid0000084004_2side.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENTeesTanksid0000512402_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENTeesTanksid0000512402_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENTeesTanksid0000512402_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENTeesTanksid0000512402_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENTeesTanksid0000512402_7additional.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENTeesTanksid0000512402_7additional.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENDressesid0000689802_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENDressesid0000689802_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENDressesid0000689802_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENDressesid0000689802_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENDressesid0000689802_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENDressesid0000766701_4full.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENDressesid0000528102_1front.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENDressesid0000528102_1front.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENDressesid0000528102_1front.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENDressesid0000528102_1front.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENDressesid0000528102_1front.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENDressesid0000528102_1front.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/input_fasionWOMENBlousesShirtsid0000299703_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/GT_fasionWOMENBlousesShirtsid0000299703_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_1/fasionWOMENBlousesShirtsid0000299703_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_2/fasionWOMENBlousesShirtsid0000299703_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/fasionWOMENBlousesShirtsid0000299703_3back.png}&
\includegraphics[height=0.24\columnwidth]{./figures/sup/comp/supp_3/att_fasionWOMENBlousesShirtsid0000299703_3back.png}
\\

 \end{tabular}}
   \vspace{-0.4cm} 
   \caption{Additional qualitative results on the DeepFashion dataset.}
   \label{fig:fashionAdd}
  \end{figure*}


==> implementation.tex <==

\subsection{Implementation details}
\label{sec:impDetails}

Even if there is no constraint on the  cardinality of the source images $M_n$  during training, in order to simplify the implementation, we train and test our networks using different steps, each step having $M_n$ fixed for all $\mathcal{X}_n$ in  $\mathcal{X}$. \enver{pay attention to this: it's very critical because the reviewers can think that all our emphasis on having $M_n$ variable in practice it is not that true... Plus, I'm not sure what I wrote is correct} %???
Specifically, we initially train $E$, $A$ and $D$ with $M_n = 2$. \enver{what about single-source exp. in which $M_n = 1$???}
Then, $A$ and $D$ are fine-tuned with $M_n = k$, where $k$ varies depending on the different experiments shown in Sec. ???.
Similarly, at testing time, we use  $M_n = k$ corresponding to value used in the fine-tuning step.


\enver{I've not read what follows from now on, which I leave for you.}
We train $G$ and $D$ for 60k iterations, with the Adam optimizer (learning rate: $2 * 10^{-4}$, $\beta_1 = 0.5$, $\beta_2 =0.999$). We use instance normalization \cite{DBLP:journals/corr/UlyanovVL16} as recommended in \cite{pix2pix2016} w. 
In the following we denote with: 
(1) $C_m^s$  a convolution layer with ReLU activation with $m$ filters and stride $s$,
(2)  $CN_m^s$  the same layer as $C_m^s$ with instance normalization before ReLU and
(3) $CD_m^s$ the same as $CN_m^s$  with the addition of dropout at rate $50\%$.

Both the source stream and transformation stream decoders have the following architecture is given by:
$CN_{64}^1 - CN_{128}^2 - CN_{256}^2 - CN_{512}^2 - CN_{512}^2 - CN_{512}^2$.
\noindent
The decoder is composed of the following convolution layers. 
$CD_{512}^2 - CD_{512}^2 - CD_{512}^2 - CN_{256}^2 - CN_{128}^2 - C_{3}^1$.
\noindent
In the last decoder layer,  the ReLU activation is replaced with $tanh$.
We employ the same discriminator architecture than in \cite{siarohin2018deformable}
In order to handle the higher resolution of the DeepFashion dataset, we add one additional convolution block ($CN_{512}^2$) to 
 the encoder (both streams) and to the decoder.


==> marketSup.tex <==
\begin{figure*}[h]
   \centering
   \setlength\tabcolsep{1.0pt}
   \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc|c}
     %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
     $x^i,i\in[1..5]$ & $x_\tau$ & $M_n=2$ & $M_n=3$ & $M_n=5$ & \small Attention Saliency\\ 

\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0036_c5s1_004401_03.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0036_c5s1_004401_03.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0036_c5s1_004401_03.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0036_c5s1_004401_03.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0036_c5s1_004401_03.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0036_c5s1_004401_03.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0608_c3s2_033087_04.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0608_c3s2_033087_04.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0608_c3s2_033087_04.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0608_c3s2_033087_04.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0608_c3s2_033087_04.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0608_c3s2_033087_04.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0996_c3s2_132669_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0996_c3s2_132669_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0996_c3s2_132669_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0996_c3s2_132669_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0996_c3s2_132669_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0996_c3s2_132669_06.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0980_c2s2_122552_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0980_c2s2_122552_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0980_c2s2_122552_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0980_c2s2_122552_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0980_c2s2_122552_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0980_c2s2_122552_06.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0133_c2s1_022601_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0133_c2s1_022601_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0133_c2s1_022601_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0133_c2s1_022601_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0133_c2s1_022601_06.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0133_c2s1_022601_06.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1429_c1s6_020496_01.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1429_c1s6_020496_01.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1429_c1s6_020496_01.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1429_c1s6_020496_01.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1429_c1s6_020496_01.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1429_c1s6_020496_01.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0094_c6s1_015851_01.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0094_c6s1_015851_01.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0094_c6s1_015851_01.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0094_c6s1_015851_01.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0094_c6s1_015851_01.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0094_c6s1_015851_01.png}
\\
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0993_c2s2_124802_03.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0993_c2s2_124802_03.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0993_c2s2_124802_03.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0993_c2s2_124802_03.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0993_c2s2_124802_03.png}&
\includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0993_c2s2_124802_03.png}
 \end{tabular}}
   \vspace{-0.4cm} 
   \caption{Additional qualitative results on the Market-1501 dataset.}
   \label{fig:qualAdd}
  \end{figure*}

%% \begin{figure*}[h]
%%    \centering
%%    \setlength\tabcolsep{1.0pt}
%%    \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc|c}
%%      %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
%%      $x^i,i\in[1..5]$ & $x_\tau$ & $M_n=2$ & $M_n=3$ & $M_n=5$ & \small Attention Saliency\\ 


%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0819_c5s2_102602_01.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0819_c5s2_102602_01.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0819_c5s2_102602_01.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0819_c5s2_102602_01.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0819_c5s2_102602_01.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0819_c5s2_102602_01.png}
%% \\
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1090_c6s3_094192_03.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1090_c6s3_094192_03.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1090_c6s3_094192_03.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1090_c6s3_094192_03.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1090_c6s3_094192_03.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1090_c6s3_094192_03.png}
%% \\
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1262_c5s3_023390_04.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1262_c5s3_023390_04.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1262_c5s3_023390_04.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1262_c5s3_023390_04.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1262_c5s3_023390_04.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1262_c5s3_023390_04.png}
%% \\
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0004_c6s3_089492_01.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0004_c6s3_089492_01.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0004_c6s3_089492_01.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0004_c6s3_089492_01.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0004_c6s3_089492_01.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0004_c6s3_089492_01.png}
%% \\
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1436_c5s3_073337_02.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1436_c5s3_073337_02.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1436_c5s3_073337_02.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1436_c5s3_073337_02.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1436_c5s3_073337_02.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1436_c5s3_073337_02.png}
%% \\
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0692_c3s2_067403_05.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0692_c3s2_067403_05.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0692_c3s2_067403_05.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0692_c3s2_067403_05.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0692_c3s2_067403_05.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0692_c3s2_067403_05.png}
%% \\
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0091_c3s1_013976_05.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0091_c3s1_013976_05.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0091_c3s1_013976_05.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0091_c3s1_013976_05.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0091_c3s1_013976_05.png}&
%% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0091_c3s1_013976_05.png}
%% \\
%%  \end{tabular}}
%%    \vspace{-0.4cm} 
%%   \caption{Caption} 
%%   \end{figure*}
%% %% \begin{figure*}[h]
%% %%    \centering
%% %%    \setlength\tabcolsep{1.0pt}
%% %%    \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc|c}
%% %%      %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
%% %%      $x^i,i\in[1..5]$ & $x_\tau$ & $M_n=2$ & $M_n=3$ & $M_n=5$ & \small Attention Saliency\\ 

%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0161_c2s2_149727_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0161_c2s2_149727_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0161_c2s2_149727_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0161_c2s2_149727_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0161_c2s2_149727_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0161_c2s2_149727_02.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0672_c6s2_056793_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0672_c6s2_056793_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0672_c6s2_056793_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0672_c6s2_056793_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0672_c6s2_056793_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0672_c6s2_056793_01.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0602_c6s2_011018_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0602_c6s2_011018_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0602_c6s2_011018_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0602_c6s2_011018_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0602_c6s2_011018_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0602_c6s2_011018_04.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1476_c3s3_078594_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1476_c3s3_078594_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1476_c3s3_078594_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1476_c3s3_078594_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1476_c3s3_078594_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1476_c3s3_078594_04.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0285_c3s1_062717_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0285_c3s1_062717_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0285_c3s1_062717_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0285_c3s1_062717_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0285_c3s1_062717_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0285_c3s1_062717_03.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1484_c6s3_090867_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1484_c6s3_090867_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1484_c6s3_090867_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1484_c6s3_090867_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1484_c6s3_090867_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1484_c6s3_090867_03.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0174_c5s1_053376_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0174_c5s1_053376_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0174_c5s1_053376_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0174_c5s1_053376_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0174_c5s1_053376_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0174_c5s1_053376_02.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0041_c5s3_075987_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0041_c5s3_075987_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0041_c5s3_075987_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0041_c5s3_075987_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0041_c5s3_075987_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0041_c5s3_075987_05.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1065_c2s2_145927_09.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1065_c2s2_145927_09.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1065_c2s2_145927_09.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1065_c2s2_145927_09.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1065_c2s2_145927_09.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1065_c2s2_145927_09.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1022_c6s2_124718_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1022_c6s2_124718_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1022_c6s2_124718_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1022_c6s2_124718_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1022_c6s2_124718_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1022_c6s2_124718_02.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0229_c3s1_046376_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0229_c3s1_046376_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0229_c3s1_046376_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0229_c3s1_046376_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0229_c3s1_046376_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0229_c3s1_046376_05.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0827_c3s2_105178_07.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0827_c3s2_105178_07.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0827_c3s2_105178_07.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0827_c3s2_105178_07.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0827_c3s2_105178_07.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0827_c3s2_105178_07.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1089_c5s3_087887_06.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1089_c5s3_087887_06.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1089_c5s3_087887_06.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1089_c5s3_087887_06.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1089_c5s3_087887_06.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1089_c5s3_087887_06.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0521_c1s2_071621_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0521_c1s2_071621_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0521_c1s2_071621_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0521_c1s2_071621_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0521_c1s2_071621_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0521_c1s2_071621_03.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0226_c3s1_047001_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0226_c3s1_047001_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0226_c3s1_047001_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0226_c3s1_047001_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0226_c3s1_047001_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0226_c3s1_047001_05.png}
%% %% \\
%% %%  \end{tabular}}
%% %%    \vspace{-0.4cm} 
%% %%   \caption{Caption} 
%% %%   \end{figure*}
%% %% \begin{figure*}[h]
%% %%    \centering
%% %%    \setlength\tabcolsep{1.0pt}
%% %%    \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc|c}
%% %%      %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
%% %%      $x^i,i\in[1..5]$ & $x_\tau$ & $M_n=2$ & $M_n=3$ & $M_n=5$ & \small Attention Saliency\\ 

%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1087_c6s3_008317_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1087_c6s3_008317_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1087_c6s3_008317_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1087_c6s3_008317_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1087_c6s3_008317_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1087_c6s3_008317_01.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0937_c3s2_118119_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0937_c3s2_118119_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0937_c3s2_118119_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0937_c3s2_118119_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0937_c3s2_118119_04.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0937_c3s2_118119_04.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0186_c3s1_039526_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0186_c3s1_039526_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0186_c3s1_039526_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0186_c3s1_039526_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0186_c3s1_039526_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0186_c3s1_039526_01.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1009_c1s4_070336_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1009_c1s4_070336_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1009_c1s4_070336_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1009_c1s4_070336_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1009_c1s4_070336_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1009_c1s4_070336_03.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1323_c3s3_052778_07.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1323_c3s3_052778_07.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1323_c3s3_052778_07.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1323_c3s3_052778_07.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1323_c3s3_052778_07.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1323_c3s3_052778_07.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0005_c3s2_088578_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0005_c3s2_088578_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0005_c3s2_088578_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0005_c3s2_088578_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0005_c3s2_088578_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0005_c3s2_088578_02.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0924_c6s2_109418_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0924_c6s2_109418_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0924_c6s2_109418_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0924_c6s2_109418_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0924_c6s2_109418_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0924_c6s2_109418_03.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0137_c5s1_024551_06.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0137_c5s1_024551_06.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0137_c5s1_024551_06.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0137_c5s1_024551_06.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0137_c5s1_024551_06.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0137_c5s1_024551_06.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0684_c3s2_064203_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0684_c3s2_064203_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0684_c3s2_064203_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0684_c3s2_064203_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0684_c3s2_064203_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0684_c3s2_064203_05.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1282_c2s3_021007_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1282_c2s3_021007_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1282_c2s3_021007_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1282_c2s3_021007_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1282_c2s3_021007_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1282_c2s3_021007_02.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0320_c2s3_074527_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0320_c2s3_074527_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0320_c2s3_074527_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0320_c2s3_074527_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0320_c2s3_074527_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0320_c2s3_074527_02.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1410_c1s6_017171_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1410_c1s6_017171_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1410_c1s6_017171_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1410_c1s6_017171_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1410_c1s6_017171_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1410_c1s6_017171_01.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0835_c3s2_106378_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0835_c3s2_106378_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0835_c3s2_106378_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0835_c3s2_106378_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0835_c3s2_106378_05.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0835_c3s2_106378_05.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1361_c2s3_035907_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1361_c2s3_035907_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1361_c2s3_035907_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1361_c2s3_035907_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1361_c2s3_035907_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1361_c2s3_035907_01.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0165_c2s1_029676_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0165_c2s1_029676_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0165_c2s1_029676_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0165_c2s1_029676_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0165_c2s1_029676_03.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0165_c2s1_029676_03.png}
%% %% \\
%% %%  \end{tabular}}
%% %%    \vspace{-0.4cm} 
%% %%   \caption{Caption} 
%% %%   \end{figure*}
%% %% \begin{figure*}[h]
%% %%    \centering
%% %%    \setlength\tabcolsep{1.0pt}
%% %%    \resizebox{0.99\textwidth}{!}{\begin{tabular}{c|c|ccc|c}
%% %%      %% &&\multicolumn{4}{c|}{Market-1501}&\multicolumn{2}{c}{DeepFashion}\
%% %%      $x^i,i\in[1..5]$ & $x_\tau$ & $M_n=2$ & $M_n=3$ & $M_n=5$ & \small Attention Saliency\\ 

%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_1310_c6s3_067892_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_1310_c6s3_067892_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/1310_c6s3_067892_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/1310_c6s3_067892_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/1310_c6s3_067892_02.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_1310_c6s3_067892_02.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0978_c6s2_117843_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0978_c6s2_117843_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0978_c6s2_117843_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0978_c6s2_117843_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0978_c6s2_117843_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0978_c6s2_117843_01.png}
%% %% \\
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/input_0650_c2s2_031262_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/GT_0650_c2s2_031262_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_2/0650_c2s2_031262_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_3/0650_c2s2_031262_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/0650_c2s2_031262_01.png}&
%% %% \includegraphics[height=0.24\columnwidth]{./figures/marketsupp_tr_5/att_0650_c2s2_031262_01.png}
%% %% \\
%% %%  \end{tabular}}
%% %%    \vspace{-0.4cm} 
%% %%   \caption{Caption} 
%% %%   \end{figure*}

